Dynkin Graphs, Gabri\'{e}lov Graphs and Triangle Singularities

Fourteen kinds of triangle singularities with modality one in Arnold's classification list are discussed. We consider which kinds of combinations of rational double points can appear on small deformation fibers of the singularities. We show that possible combinations of rational double points can be described by a unique principle from the view point of Dynkin graphs.

==> Read_Me_96wall.tex <==
%auto-ignore
You may need erase the comment symbol "%" before \psfigdriver and
rewrite the argument of \psfigdriver depending on your driver.
See page 317 of "The LaTeX Cpmpanion."

To reproduce this manuscript the following files are necessary:

(LaTeX2e files by myself)
96wall.tex
(Graphic files by myself--Macintosh Encapsulated PostScript format)
wall_fig1.eps
wall_fig2.eps
wall_fig3.eps
wall_fig4.eps
wall_fig5.eps
wall_fig6.eps
(Standard files)
amsart.cls    1995/02/01 v1.2a
amsgen.sty    1995/01/31 v1.2a
amsmath.sty    1995/02/01 v1.2a AMS math features
amstext.sty    1995/01/25 v1.2
amsbsy.sty    1995/01/20 v1.2
amsopn.sty    1995/01/20 v1.2 operator names
amsfonts.sty    
amsthm.sty    1995/02/01 v1.2a
epsfig.sty    1994/06/07 1.3
graphicx.sty    1994/05/30 v0.4b
keyval.sty    1994/02/01 v1.06, 1994/03/15 v1.07
graphics.sty    1994/10/24 v0.5d
trig.sty    1994/03/15 v1.07
graphics.cfg
dvips.def    1994/06/08 v1.6 
textures.def.tex    textures.def Graphics extensions
Umsa.fd    1994/05/12 v2.2b Standard AMS font definitions
Umsb.fd    1994/05/12 v2.2b Standard AMS font definitions
\end{filecontents}
